Efficient Natural Gradient Descent Methods for Large-Scale PDE-Based Optimization Problems

We propose efficient numerical schemes for implementing the natural gradient descent (NGD) for a broad range of metric spaces with applications to PDE-based optimization problems. Our technique represents the natural gradient direction as a solution to a standard least-squares problem. Hence, instead of calculating, storing, or inverting the information matrix directly, we apply efficient methods from numerical linear algebra. We treat both scenarios where the Jacobian, i.e., the derivative of the state variable with respect to the parameter, is either explicitly known or implicitly given through constraints. We can thus reliably compute several natural NGDs for a large-scale parameter space. In particular, we are able to compute Wasserstein NGD in thousands of dimensions, which was believed to be out of reach. Finally, our numerical results shed light on the qualitative differences between the standard gradient descent and various NGD methods based on different metric spaces in nonconvex optimization problems.

==> arXiv v3/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here


% \usepackage{refcheck}
% %%% Infrastructure    
% \makeatletter
% \newcommand{\refcheckize}[1]{%
%   \expandafter\let\csname @@\string#1\endcsname#1%
%   \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[1]{%
%     \csname @@\string#1\endcsname{##1}\wrtusdrf{##1}}%
%   \expandafter\let\expandafter#1\csname relax\string#1\endcsname
% }
% \makeatother
% %%%
% %%% Now we add the reference commands we want refcheck to be aware of
% \refcheckize{\cref}
% \refcheckize{\Cref}


\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{booktabs}       % professional-quality tables
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{algorithmicx}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

%\smartqed  % flush right qed marks, e.g. at end of proof
%
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage[shortlabels]{enumitem}
\usepackage{subfig}
\usepackage{epstopdf}
% \setlength {\marginparwidth }{2cm}
\usepackage{todonotes}
\usepackage{hyperref}
\usepackage{comment}
% \usepackage{mathptmx}  
% \usepackage[margin=3cm]{geometry}
\usepackage[normalem]{ulem}
\usepackage{pifont}% http://ctan.org/pkg/pifont


\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\Pp}{\mathcal{P}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\M}{\mathcal{M}}
\DeclareMathOperator{\diag}{diag}
\newcommand*\Laplace{\mathop{}\!\mathbin\bigtriangleup}
\newcommand\sbullet[1][.5]{\mathbin{\vcenter{\hbox{\scalebox{#1}{$\bullet$}}}}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\magenta}[1]{\textcolor{magenta}{#1}}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
\newsiamthm{proposition}{Proposition}

% Sets running headers as well as PDF title and authors
\headers{Efficient Natural Gradient Descent Methods}{L. Nurbekyan, W. Lei, and Y. Yang}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.

% \title{Efficient Natural Gradient Descent Methods for Large-Scale Optimization Problems\thanks{Submitted to the editors on \today.
\title{Efficient Natural Gradient Descent Methods for Large-Scale PDE-Based Optimization Problems\thanks{Submitted to the editors. %on \today.
\funding{L.~Nurbekyan was partially supported by AFOSR MURI FA 9550 18-1-0502 grant. Y.~Yang was partially supported by NSF grant DMS-1913129.}}}

% Authors: full names plus addresses.
\author{
Levon Nurbekyan\thanks{Department of Mathematics, UCLA (\email{lnurbek@math.ucla.edu}).}
\and Wanzhou Lei\thanks{Harvard University (\email{wanzhoulei@g.harvard.edu}).}
\and Yunan Yang\thanks{Institute for Theoretical Studies, ETH Z\"urich (\email{yunan.yang@eth-its.ethz.ch}).}
}

\usepackage{amsopn}



%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

